Adding Time to Pushdown Automata

In this tutorial, we illustrate through examples how we can combine two classical models, namely those of pushdown automata (PDA) and timed automata, in order to obtain timed pushdown automata (TPDA). Furthermore, we describe how the reachability problem for TPDAs can be reduced to the reachability problem for PDAs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{U. Fahrenberg, A. Legay and C. Thrane: \\
Quantities in Formal Methods (QFM 2012)\\
EPTCS 103, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.103.1}{10.4204/EPTCS.103.1}}

